Predicting score distribution to improve non-intrusive speech quality estimation

Deep noise suppressors (DNS) have become an attractive solution to remove background noise, reverberation, and distortions from speech and are widely used in telephony/voice applications. They are also occasionally prone to introducing artifacts and lowering the perceptual quality of the speech. Subjective listening tests that use multiple human judges to derive a mean opinion score (MOS) are a popular way to measure these models' performance. Deep neural network based non-intrusive MOS estimation models have recently emerged as a popular cost-efficient alternative to these tests. These models are trained with only the MOS labels, often discarding the secondary statistics of the opinion scores. In this paper, we investigate several ways to integrate the distribution of opinion scores (e.g. variance, histogram information) to improve the MOS estimation performance. Our model is trained on a corpus of 419K denoised samples by 320 different DNS models and model variations and evaluated on 18K test samples from DNSMOS. We show that with very minor modification of a single task MOS estimation pipeline, these freely available labels can provide up to a 0.016 RMSE and 1% SRCC improvement.

==> sections/abstract.tex <==
\begin{abstract}

In this paper, we investigate and develop a deep neural network-based model to estimate the subjective quality of speech signals processed by a deep noise suppression (DNS) model.
DNS models have become an attractive solution to remove background noise, reverberation, and distortions from speech and are widely used in telephony and voice applications. 
However, these DNS models may also introduce artifacts that lower the perceptual quality of the speech. Employing subjective listening tests to measure perceptual quality can be tedious and expensive. 
We develop a convolutional LSTM based model to predict the mean opinion score (MOS) of speech signals preprocessed by various DNS models.
We investigate the efficacy of incorporating the distribution of the subjective scores to improve the MOS estimation performance using multi-task learning. 
Our MOS estimation model is trained on a corpus of 419K de-noised samples and evaluated on 18K
validation samples processed by 320 different DNS models and model variations. 
Our experimental results indicate that using score distribution in addition to MOS labels can improve MOS estimation performance. 
%Our best-performing model achieves a stacked ranked correlation of 0.98 and an RMSE of 0.10.
\end{abstract}

==> tables/results-old.tex <==
\begin{table*}[!htb]
\caption{Comparison of Model Performance (MOS\_E/418K samples)}
\label{tab:results}
\resizebox{\linewidth}{!}{%
\begin{tabular}{@{}lllllllll@{}}
\toprule
\multicolumn{1}{c}{\multirow{2}{*}{Model}} &
  \multicolumn{1}{c}{\multirow{2}{*}{Task Type}} &
  \multicolumn{1}{c}{\multirow{2}{*}{Ground Truth Labels}} &
  \multicolumn{3}{c}{Per-file} &
  \multicolumn{3}{c}{Stack   Ranked} \\ \cmidrule(l){4-9} 
\multicolumn{1}{c}{} &
  \multicolumn{1}{c}{} &
  \multicolumn{1}{c}{} &
  \multicolumn{1}{c}{Correlation} &
  \multicolumn{1}{c}{MAE} &
  \multicolumn{1}{c}{RMSE} &
  \multicolumn{1}{c}{Correlation} &
  \multicolumn{1}{c}{MAE} &
  \multicolumn{1}{c}{RMSE} \\ \midrule\midrule
DNSMOS                                                     & Single & MOS                       & 0.7527 & 0.4094 & 0.5247 & 0.9519 & 0.2402          & 0.2529          \\\cmidrule{1-9}
ConvLSTM (Single Task MOS Prediction)                      & Single & MOS                       & 0.7655 & 0.3735 & 0.4787 & 0.9769 & 0.0850          & 0.1205          \\\cmidrule{1-9}
ConvLSTM (Multi Task MOS and Std Dev of Scores Prediction) & Multi  & MOS + StdDev of  Scores   & 0.7668 & 0.3749 & 0.4779 & \textbf{0.9829} & 0.0787          & 0.1130          \\\cmidrule{1-9}
ConvLSTM + Inverse Variance Weighting                      & Single & MOS                       & 0.7022 &        &        &        &                 &                 \\\cmidrule{1-9}
ConvLSTM + Linear Variance Weighting                       & Single & MOS                       & 0.7656 &        &        &        &                 &                 \\\cmidrule{1-9}
ConvLSTM + Predict 5 Opinion Scores                                 & Multi  & MOS + StdDev of Scores    & \textbf{0.7747} & \textbf{0.3631} & \textbf{0.4635} & 0.9797 & \textbf{0.0716} & \textbf{0.1042} \\\cmidrule{1-9}
ConvLSTM + Predict 5 Opinion Scores (w Sigmoid activation)          & Multi  & MOS + StdDev of Scores    & 0.7710 & 0.3685 & 0.4709 & 0.9711 & 0.0870          & 0.1169          \\\cmidrule{1-9}
ConvLSTM + Histogram prediction (Cross Entropy Loss)       & Multi  & 5 Bin Histogram of Scores & 0.7661 & 0.3712 & 0.4730 & 0.9724 & 0.0730          & 0.1044          \\\cmidrule{1-9}
ConvLSTM  + Histogram prediction (EMD/Wasserstein Loss)    & Multi  & 5 Bin Histogram of Scores & 0.7633 &        &        &        &                 &                 \\\cmidrule{1-9}
ConvLSTM  + Histogram prediction (Chi Square)              & Multi  & 5 Bin Histogram of Scores & 0.7577 &        &        &        &                 &                 \\\cmidrule{1-9}
ConvLSTM  + Median of the Opinion Scores                            & Multi  & MOS + Median of Scores    & 0.7720 &        &        &        &                 &                 \\\cmidrule{1-9}
\begin{tabular}[c]{@{}l@{}}ConvLSTM \\ + MOS prediction with confident labels (StdDev of Scores$<=$1)\end{tabular} &
  Multi &
  5 Bin Histogram of Scores &
  0.7605 &
   &
   &
   &
   &
   \\ \bottomrule
\end{tabular}
}
\end{table*}

==> tables/results.tex <==
\begin{table*}[!htb]
\centering
\caption{Comparison of Model Performance}
% (MOS\_E/418K samples)
\label{tab:results}
\resizebox{\textwidth}{!}{%
\begin{tabular}{@{}llllcccccc@{}}
\toprule
\multicolumn{1}{c}{\multirow{2}{*}{Model}} & \multicolumn{1}{c}{\multirow{2}{*}{Task}} & \multicolumn{1}{c}{\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Ground Truth \\ Labels\end{tabular}}} & \multicolumn{1}{c}{\multirow{2}{*}{Loss}} & \multicolumn{3}{c}{Per-file} & \multicolumn{3}{c}{Stack Ranked} \\ \cmidrule(l){5-10} 
\multicolumn{1}{c}{} & \multicolumn{1}{c}{} & \multicolumn{1}{c}{} & \multicolumn{1}{c}{} & $\rho$ & MAE & RMSE & $\rho$ & MAE & RMSE \\ \midrule
DNSMOS & Single & MOS &  & 0.7527 & 0.4094 & 0.5247 & 0.9519 & 0.2402 & 0.2529 \\
ConvLSTM & Single & MOS & MSE & 0.7655 & 0.3735 & 0.4787 & 0.9769 & 0.0850 & 0.1205 \\
ConvLSTM (Multi Task MOS and $\sigma$ Prediction) & Multi & MOS, $\sigma$ & MSE & 0.7668 & 0.3749 & 0.4779 & \textbf{0.9829} & 0.0787 & 0.1130 \\
ConvLSTM + Inverse Variance Weighting & Single & MOS & MSE & 0.7022 &  &  &  &  &  \\
ConvLSTM + Linear Variance Weighting & Single & MOS & MSE & 0.7656 &  &  &  &  &  \\
ConvLSTM + Predict 5 Opinion Scores & Multi & MOS + $\sigma$ & MSE & \textbf{0.7747} & \textbf{0.3631} & \textbf{0.4635} & 0.9797 & \textbf{0.0716} & \textbf{0.1042} \\
ConvLSTM + Predict 5 Opinion Scores + Sigmoid activation) & Multi & MOS + $\sigma$ & MSE & 0.7710 & 0.3685 & 0.4709 & 0.9711 & 0.0870 & 0.1169 \\
ConvLSTM + Histogram prediction & Multi & Histogram & Cross Entropy & 0.7661 & 0.3712 & 0.4730 & 0.9724 & 0.0730 & 0.1044 \\
ConvLSTM + Histogram prediction & Multi & Histogram & Wasserstein & 0.7633 &  &  &  &  &  \\
ConvLSTM + Histogram prediction & Multi & Histogram & Chi Square & 0.7577 &  &  &  &  &  \\
ConvLSTM + Median of the Opinion Scores & Multi & MOS + Median & MSE & 0.7720 &  &  &  &  &  \\
% ConvLSTM + MOS prediction with confident labels ($\sigma<=$1) & Multi & Histogram & MSE & 0.7605 &  &  &  &  &  \\ 
\bottomrule
\end{tabular}%
}
\end{table*}
